X-DFS: Explainable Artificial Intelligence Guided Design-for-Security Solution Space Exploration

Design and manufacturing of integrated circuits predominantly use a globally distributed semiconductor supply chain involving diverse entities. The modern semiconductor supply chain has been designed to boost production efficiency, but is filled with major security concerns such as malicious modifications (hardware Trojans), reverse engineering (RE), and cloning. While being deployed, digital systems are also subject to a plethora of threats such as power, timing, and electromagnetic (EM) side channel attacks. Many Design-for-Security (DFS) solutions have been proposed to deal with these vulnerabilities, and such solutions (DFS) relays on strategic modifications (e.g., logic locking, side channel resilient masking, and dummy logic insertion) of the digital designs for ensuring a higher level of security. However, most of these DFS strategies lack robust formalism, are often not human-understandable, and require an extensive amount of human expert effort during their development/use. All of these factors make it difficult to keep up with the ever growing number of microelectronic vulnerabilities. In this work, we propose X-DFS, an explainable Artificial Intelligence (AI) guided DFS solution-space exploration approach that can dramatically cut down the mitigation strategy development/use time while enriching our understanding of the vulnerability by providing human-understandable decision rationale. We implement X-DFS and comprehensively evaluate it for reverse engineering threats (SAIL, SWEEP, and OMLA) and formalize a generalized mechanism for applying X-DFS to defend against other threats such as hardware Trojans, fault attacks, and side channel attacks for seamless future extensions.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sc.tex <==
\section{\textcolor{blue}{Extending X-DFS for Side Channel Defense}\label{sec:xdfs_schannel}}
\textcolor{blue}{In this section we will extend X-DFS for supporting power side channel leakage defense and showcase quantitative experimental results to support its efficacy.}

% \subsection{}
\subsection{\textcolor{blue}{Power Leakage Estimator Tool: TVLA}}
\textcolor{blue}{As a metric for estimating power side channel leakage, we decided to go with the Test Vector Leakage Assessment (TVLA) approach. The TVLA methodology uses Welch’s T-test to evaluate the security of cryptographic implementations against side-channel attacks \cite{schneider2016leakage, sadhukhan2023valiant}. The t-statistic is computed using the mean, standard deviation, and cardinality of these sets. Let $Q_0$ and $Q_1$ denote two sets of side-channel traces that are independent and need to be tested. Let $\mu_0$, $\mu_1$ represent the mean, $\rho_0$, $\rho_1$ represent the standard deviation, and $n_0$, $n_1$ represent the cardinality of set $Q_0$, $Q_1$. Then, $t$ will be computed as shown in Eqn.~\ref{eqn_tvla}.} 

% VALIANT \cite{sadhukhan2023valiant} is an EDA tool-flow that operates on gate-level designs to identify and mitigate side-channel leakages. VALIANT performs power simulation and leakage evaluation using the Test Vector Leakage Assessment (TVLA) method.  

% Side-channel attacks exploit physical characteristics like power consumption to leak information from cryptographic devices. These are significant threats, necessitating robust evaluation methodologies. Schneider et al. \cite{schneider2016leakage} addresses the need for a standardized approach to evaluate the side-channel vulnerabilities of cryptographic devices. They focus on the use of Welch’s t-test for leakage assessment and provides a comprehensive methodology for its application, particularly in higher-order and multivariate settings. Welch’s t-test is proposed for its simplicity and independence from device architecture, aiding in detecting any type of leakage \cite{schneider2016leakage}. 
% The Test Vector Leakage Assessment (TVLA) methodology uses Welch’s T-test to evaluate the security of cryptographic implementations against side-channel attacks \cite{sadhukhan2023valiant}. VALIANT \cite{sadhukhan2023valiant} is an EDA tool-flow that operates on gate-level designs to identify and mitigate side-channel leakages. VALIANT performs power simulation and leakage evaluation using the Test Vector Leakage Assessment (TVLA) method. TVLA's advantage lies in its independence from any specific leakage model and its straightforward extensions for higher-order leakage assessments \cite{sadhukhan2023valiant}. The t-statistic is computed using the mean, standard deviation, and cardinality of these sets. Let $Q_0$ and $Q_1$ denote two sets of side-channel traces that are independent and need to be tested. Let $\mu_0$, $\mu_1$ represent the mean, $\rho_0$, $\rho_1$ represent the standard deviation, and $n_0$, $n_1$ represent the cardinality of set $Q_0$, $Q_1$. Then, $t$ will be: }

\begin{equation}
\label{eqn_tvla}
\textcolor{blue}{t = \frac{\mu_0 - \mu_1}{\sqrt{\frac{\rho_0^2}{n_0} + \frac{\rho_1^2}{n_1}}}}
\end{equation}

% \textcolor{blue}{In previous studies on logic locking, SAIL has been employed as an indicator that guides us in extracting the structural information from a design and constructing a knowledge base that is utilized by machine learning models.  For this task, we employ TVLA as our main indicator to facilitate the creation of a knowledge base, similar to what SAIL did. Finally, our predictive models utilize this knowledge base.
% }
\subsection{\textcolor{blue}{Side Channel Countermeasure: Masking}}
 \textcolor{blue}{
 % Numerous significant hardware countermeasure \cite{das2018asni}, \cite{sasdrich2015side} strategies have been presented to prevent side channel attacks. However, among these schemes, 
 Masking \cite{trichina2003combinational}, \cite{gross2016domain} has emerged as the most popular and frequently adopted countermeasure for power side channel leakage. The fundamental concept of masking is introducing randomness into the execution of sensitive information during a cryptographic operation. 
 % This is accomplished by implementing a secret sharing scheme at the logic level \cite{shamir1979share}. 
 To mitigate side channel threats, we employ a method described by Trichina et. al. \cite{trichina2003combinational} that enables secure calculation of binary AND operations on masked data, ensuring the concealment of actual data bits. 
 % Trichina \cite{trichina2003combinational} introduces a combinational logic design to perform masked AND operations, ensuring that intermediate results do not compromise security.
 }
\input{Algo/gen_schannel} 
\input{Algo/ai_schannel} 
\input{Table/coreResult_PSChannel}
% \input{Table/coreResult_PSChannel_RF}
\input{Table/coreResult_PSChannel_two}
\subsection{\textcolor{blue}{X-DFS Methodology: Power Side Channel}}
\textcolor{blue}{We have expanded our X-DFS in order to mitigate power side channel vulnerabilities, while keeping the underlying methodology same (see Fig.~\ref{fig:overview}). 
% The process of creating a knowledge base remains unchanged from our previously stated technique in Fig.~\ref{fig:overview}.
Here our DFS constructs are the masking gates proposed by Trichina et. al. \cite{trichina2003combinational}. Our evaluation metric is TVLA. The process of knowledge extraction is shown in Algo.~\ref{algo:knowledge_extraction_sc} and the process of X-DFS guided masking is shown in Algo.~\ref{algo:xdfs_leakage}}.   
% Similarly, it involves using random DFS insertion attempts to understand what mitigation approachs works best, employing XAI models to learn and collect information, and extracting rules from the XAI model. 
% We have shown two algorithms (Algo.~\ref{algo:knowledge_extraction_sc}, Algo.~\ref{algo:xdfs_leakage}) for this expanded task. The basic variations and commonalities with prior algorithms are apparent here.}

\textcolor{blue}{Algo.~\ref{algo:knowledge_extraction_sc} takes as input the digital design ($design$), number of gates to mask ($modSize$), structural feature locality size ($loc$), an iteration threshold for termination ($Th_{it}$), and a masking good threshold ($Th_r$). In line 1, we analyze the input design and extract the information using an internal graph data structure. In line 2, we obtain the leakage information of all gates by executing TVLA. In lines 7-22, we make alterations to the design, obtain the leakage value once more, compare it, and continue this process until a termination condition is satisfied. This terminating condition might be a user-specified iteration limit ($Th_{it}$) or the unavailability of gates for selection, as shown in line 22. In line 8, we alter the design by randomly selecting gates and substituting them with the corresponding masking gates \cite{trichina2003combinational}. We select the remaining unaltered gates ($remGate$) from the updated design mentioned in line 9. The variable $remGate$ is crucial since it will be utilized in the subsequent iteration to randomly select gates.
% This procedure will continue till termination. 
% This algorithm will terminate when the $remgate$ size is smaller than the $modSize$ or certain iteration ($Th_{it}$) is met.  
Next, we get the leakage information from the altered design in line 11. At line 13, we gather the structural features of each gate based on the size of the locality ($loc$, an user input). The technique is identical to the collection of structural features for logic locking, with the only difference being that the breadth-first-search starts from the target gate being considered for masking.
% Since side channel phenomena is often independent of functional activity, we have chosen to ignore the functional feature in this study. 
In line 14, we calculate the ratio ($ratio$) and then compare it with a specific threshold value ($Th_r$, an user input). Based on this comparison, we assign a label of either 1 or 0 from line 15-18. The term $ratio$ represents the percentage of variation between the former leakage value of a gate and its post-masking leakage value and it is computed by $leak\_Comp()$ in line 14 (using Eqn.~\ref{eqn_leakage}). Here $L_P$ and $L_N$ denote the prior leakage value and the post-masking leakage value respectively, of a given gate. In line 21, the $run$ variable keeps track of the iterations and the final dataset is returned in line 23. This final dataset is used to train different AI models following similar strategies explained in Section~\ref{sec:ModelTraning}}.

\begin{equation}
\label{eqn_leakage}
\textcolor{blue}{ratio = \frac{L_A - L_B}{L_A}}
\end{equation}

% \textcolor{blue}{Setting the $Th_r$ value to 0.5 indicates that the label will be assigned as 1, which signifies a good observation for X-DFS, where there is a reduction of 50\% or more in the modified gate's leakage value compared to its previous leakage value. 

% \textcolor{blue}{In line 20, the $run$ variable keeps track of the iterations and the final dataset is returned in line 22.}

\textcolor{blue}{Algo.~\ref{algo:xdfs_leakage} describes the process of utilizing an trained X-DFS model for efficiently reducing power side channel leakage. 
% demonstrates the evaluation of X-DFS to mitigate side channel vulnerabilities by employing a trained machine learning model. 
Algo.~\ref{algo:xdfs_leakage} takes as input the digital design ($design$), trained X-DFS model ($Model$), number of gates to mask ($modSize$), structural feature locality size ($loc$), and a masking good threshold ($Th_r$). In line 1 and line 2 we build the graph from the input design and find the leakage respectively. Inside the block spanning from line 3 to line 6, we iterate through each gate in $G$. For each gate, we extract the structural features and feed them into the trained model. This process provides a prediction $P$ in the form of a real number, which is then added to the $options$ list. In line 7, we sort $options$ in descending order to obtain the top candidates for the selection. A modified design is developed using the top candidates. In line 9, we conduct a measurement of the leakage of the modified design. In line 10, we gain some insights ($info$) utilizing the $Th_r$, that are shown in the results section later.  }

\subsection{\textcolor{blue}{Experimental Setup: Power Side Channel}}
\textcolor{blue}{Algo.~\ref{algo:knowledge_extraction_sc} was utilized to extract training data from a collection of small designs (ISCAS-85, c1355, c1908, c2670, c3540, c5315, c6288, c7552 \cite{designs}) in order to speed up the learning process (similar to our logic locking case-study). During the evaluation process in Algo.~\ref{algo:xdfs_leakage}, we employ large-scale designs (such as sqrt, sin, div, arbiter, memctrl, log2, square, multiplier, voter) using a transfer learning technique to gain a deeper understanding of the scalability of the proposed framework. For both algorithms, locality size ($loc$) and threshold value ($Th_r$) were set to 5 and 0.7 respectively. $modSize$ was fixed at 200 for Algo.~\ref{algo:knowledge_extraction_sc}. For Algo.~\ref{algo:xdfs_leakage}, $modSize$ was taken as specific \% of each design size. All the experiment are run on the following computing system: Intel Core i9-11900, 8 cores and 16 threads, 32GB RAM. It takes 3 hours to generate the dataset for $Th_{it} = 30$. Finally, the optimized design is returned. For running TVLA, we have used `10000' as the number of input traces. For masking we use the follow gates from \cite{trichina2003combinational}: AND, OR, NAND, NOR.}

\textcolor{blue}{After getting the dataset, we utilize different AI algorithms to validate the approach. We have experimented with the likes of Random Forest, SVM, Regression, and Boosting. Among them, XGBoost with learning rate of 0.01 performs the best. }

\subsection{\textcolor{blue}{Results: Power Side Channel}}
\textcolor{blue}{In Table~\ref{table:psc_result} and Table~\ref{table:psc_result_xgb_two}, we have demonstrated the effectiveness of X-DFS in mitigating side channel threats. The specific settings and algorithm parameters are described in the Table headings. The `Before' and `After' columns indicate the average leakage of the chosen gates before and after the masking, respectively. The `Reduction' column represents the percentage of reduction that has occurred after the masking. `Insertion Accuracy' refers the percentage of the selected gates that experience a reducing in leakage greater than or equal to the threshold value ($Th_r$). The `Insertion Accuracy' indicates the quality of the masking process. It is evident from the `Insertion Accuracy' that the X-DFS framework leads to more optimal selection of design gates for masking. Also the overall leakage reduction is more when using X-DFS. Future works will explore the efficiency of X-DFS in terms of mitigating power side channel leakage for more: (1) settings/parameters variations; (2) AI algorithms; (3) Masking strategies; (4) Power side channel metrics/attacks}.

% We provide conclusive proof of the continuous improvement of X-DFS in effectively selecting the appropriate gates compared to random selection. $modSize$ in Algo.~\ref{algo:xdfs_leakage} takes 1\% and 2\% overhead of each design for Table~\ref{table:psc_result} and Table~\ref{table:psc_result_xgb_two} correspondingly. The 'Before' and 'After' columns indicate the average leakage of the chosen gates before and after the insertion, respectively. The 'Reduction' column represents the percentage of reduction that has occurred after the insertion. 'Insertion Accuracy' refers the percentage of number of selected gates that reduce leakage greater than or equal to the threshold value ($Th_r$).}

\input{fig_latex/sc_rules}
\input{Table/extractedRules_sc}



\subsection{\textcolor{blue}{Explainability: Rules for Side Channel defense}}
\textcolor{blue}{We build the waterfall graph using the same method as previously described. This time, the graphs are generated to extract the rules that have been used for side channel defense in Fig.~\ref{fig:add_rules_sc}. We describe these rules in Table~\ref{table:extractedRules_sc}.}

% like the following:}
% \begin{enumerate}[(i)]
        
%     \item \textcolor{blue}{For case [A], X-DFS\_Model will select the gate and replace it with corresponding masking gate to reduce the leakage if $NOT$ gate is present in gate3 ($G3$) and gate5 ($G5$) as well as gate1 ($G1$) and gate2 ($G2$) are connected.}

%     \item \textcolor{blue}{For case [B], X-DFS\_Model will avoid the gate from selecting if gate2 ($G2$) and gate3 ($G3$) are connected as well as the it does not find any $NOT$ and $OR$ gate in gate3 ($G3$) and gate2 ($G2$) respectively.}
% \end{enumerate}

